Snowmass2021 Cosmic Frontier White Paper: High Density Galaxy Clustering in the Regime of Cosmic Acceleration

Joint studies of imaging and spectroscopic samples, informed by theory and simulations, offer the potential for comprehensive tests of the cosmological model over redshifts z<1.5. Spectroscopic galaxy samples at these redshifts can be increased beyond the planned Dark Energy Spectroscopic Instrument (DESI) program by at least an order of magnitude, thus offering significantly more constraining power for these joint studies. Spectroscopic observations of these galaxies in the latter half of the 2020's and beyond would leverage the theory and simulation effort in this regime. In turn, these high density observations will allow enhanced tests of dark energy, physics beyond the standard model, and neutrino masses that will greatly exceed what is currently possible. Here, we present a coordinated program of simulations, theoretical modeling, and future spectroscopy that would enable precise cosmological studies in the accelerating epoch where the effects of dark energy are most apparent.

==> science.tex <==






``Current lensing measurements indicate tension with predictions from the CMB under a $\Lambda$CDM model, but further studies are needed to improve the precision and theoretical modeling of these measurements. By combining imaging and spectroscopy, the community can assess whether an additional field, modifications to General Relativity, or other extensions to the Standard Model are required to elucidate the nature of these tensions.''

\subsection{Growth of structure:  Probe origin of cosmic acceleration at late times}

\begin{figure}
    \centering
    \includegraphics{np1.png}
    \caption{Is some version of that plot helpful, Kyle? I just assumed Planck and $b_{\rm lin}=2$ for this version.
    {\bf KD:  yes, this looks perfect.  How easy is it to have a redshift evolving bias and to match the DESI n(z) to the as-expected n(z)?}
    }
    \label{fig:np1}
\end{figure}

\subsection{Full-shape power spectrum measurements:  constrain neutrino mass}

\subsection{Small-scale clustering: particle nature of dark matter}

\subsection{Multiple probes:  new particle or field contents in the cosmological model}
